Modeling Virus Transmission Risks in Commuting with Emerging Mobility Services: A Case Study of COVID-19

Commuting is an important part of daily life. With the gradual recovery from COVID-19 and more people returning to work from the office, the transmission of COVID-19 during commuting becomes a concern. Recent emerging mobility services (such as ride-hailing and bike-sharing) further deteriorate the infection risks due to shared vehicles or spaces during travel. Hence, it is important to quantify the infection risks in commuting. This paper proposes a probabilistic framework to estimate the risk of infection during an individual's commute considering different travel modes, including public transit, ride-share, bike, and walking. The objective is to evaluate the probability of infection as well as the estimation errors (i.e., uncertainty quantification) given the origin-destination (OD), departure time, and travel mode. We first define a general trip planning function to generate trip trajectories and probabilities of choosing different paths according to the OD, departure time, and travel mode. Then, we consider two channels of infections: 1) infection by close contact and 2) infection by touching surfaces. The infection risks are calculated on a trip segment basis. Different sources of data (such as smart card data, travel surveys, and population data) are used to estimate the potential interactions between the individual and the infectious environment. The model is implemented in the MIT community as a case study. We evaluate the commute infection risks for employees and students. Results show that most of the individuals have an infection probability close to zero. The maximum infection probability is around 0.8%, implying that the probability of getting infected during the commuting process is low. Individuals with larger travel distances, traveling in transit, and traveling during peak hours are more likely to get infected.

==> record <==
Let us divide the support of the random variable $\boldsymbol{Q}|_{\boldsymbol{x}^*}$ as three mutually exclusive subsets:
\begin{align}
 &   \mathcal{Q}({\boldsymbol{x}^*})^{\text{Leq}} = \mathcal{Q}({\boldsymbol{x}^*})\cap\{\hat{\boldsymbol{q}}:\; 0 \leq \hat{\boldsymbol{q}} < \mathbb{E}[\boldsymbol{Q}|_{\boldsymbol{x}^*}] - \boldsymbol{\epsilon}\}\\
&    \mathcal{Q}({\boldsymbol{x}^*})^{\text{Mid}} = \mathcal{Q}({\boldsymbol{x}^*})\cap\{\hat{\boldsymbol{q}}:\; \mathbb{E}[\boldsymbol{Q}|_{\boldsymbol{x}^*}] - \boldsymbol{\epsilon} \leq \hat{\boldsymbol{q}} \leq \mathbb{E}[\boldsymbol{Q}|_{\boldsymbol{x}^*}] + \boldsymbol{\epsilon}\}\\
&    \mathcal{Q}({\boldsymbol{x}^*})^{\text{Geq}} = \mathcal{Q}({\boldsymbol{x}^*})\cap\{\hat{\boldsymbol{q}}:\; \mathbb{E}[\boldsymbol{Q}|_{\boldsymbol{x}^*}] + \boldsymbol{\epsilon} < \hat{\boldsymbol{q}} \leq \boldsymbol{q}^{\text{Max}}\}
\end{align}
where $ \mathcal{Q}({\boldsymbol{x}^*}) = \mathcal{Q}({\boldsymbol{x}^*})^{\text{Leq}} \cup\mathcal{Q}({\boldsymbol{x}^*})^{\text{Mid}} \cup\mathcal{Q}({\boldsymbol{x}^*})^{\text{Geq}} $

We can calculate the summation over these three subsets separately:

\noindent \textbf{(1) Bounds on the summation over} $\mathcal{Q}({\boldsymbol{x}^*})^{\text{Leq}}$:
\begin{align}
    \sum_{\hat{\boldsymbol{q}}\in\mathcal{Q}({\boldsymbol{x}^*})^{\text{Leq}}} L\cdot\norm{\hat{\boldsymbol{q}} - \boldsymbol{q}^*}_{1} \cdot \mathbb{P}_{\boldsymbol{Q}|_{\boldsymbol{x}^*}}(\hat{\boldsymbol{q}}) 
    & \leq \sum_{\hat{\boldsymbol{q}}\in\mathcal{Q}({\boldsymbol{x}^*})^{\text{Leq}}} L\cdot\left(\norm{\hat{\boldsymbol{q}} - \mathbb{E}[\boldsymbol{Q}|_{\boldsymbol{x}^*}]}_{1} + \norm{\mathbb{E}[\boldsymbol{Q}|_{\boldsymbol{x}^*}] - \boldsymbol{q}^*}_{1}\right) \cdot \mathbb{P}_{\boldsymbol{Q}|_{\boldsymbol{x}^*}}(\hat{\boldsymbol{q}}) 
\end{align}
which is followed by the triangle inequality. Notice that
\begin{align}
& \sum_{\hat{\boldsymbol{q}}\in\mathcal{Q}({\boldsymbol{x}^*})^{\text{Leq}}} L\cdot \norm{\hat{\boldsymbol{q}} - \mathbb{E}[\boldsymbol{Q}|_{\boldsymbol{x}^*}] }_{1} \cdot \mathbb{P}_{\boldsymbol{Q}|_{\boldsymbol{x}^*}}(\hat{\boldsymbol{q}})  \leq L\cdot\sum_{\hat{\boldsymbol{q}}\in\mathcal{Q}({\boldsymbol{x}^*})^{\text{Leq}}} 
\norm{\mathbb{E}[\boldsymbol{Q}|_{\boldsymbol{x}^*}]}_1 \cdot \mathbb{P}_{\boldsymbol{Q}|_{\boldsymbol{x}^*}}(\hat{\boldsymbol{q}}) \nonumber \\
&=
L\cdot\norm{\mathbb{E}[\boldsymbol{Q}|_{\boldsymbol{x}^*}]}_1\cdot\mathbb{P}\big[ \boldsymbol{Q}|_{\boldsymbol{x}^*} \leq \mathbb{E}[\boldsymbol{Q}|_{\boldsymbol{x}^*}]  - \boldsymbol{\epsilon}\big]\leq L\cdot\norm{\mathbb{E}[\boldsymbol{Q}|_{\boldsymbol{x}^*}]}_1\cdot \norm{\boldsymbol{\Gamma}}_2^2
\label{eq_prop2_leq_0}
\end{align}
where the last inequality is the result of the following:
\begin{align}
   & \mathbb{P}\big[ \boldsymbol{Q}|_{\boldsymbol{x}^*} \leq \mathbb{E}[\boldsymbol{Q}|_{\boldsymbol{x}^*}]  - \boldsymbol{\epsilon}\big]\leq \mathbb{P}\big[ |\boldsymbol{Q}|_{\boldsymbol{x}^*} - \mathbb{E}[\boldsymbol{Q}|_{\boldsymbol{x}^*}]| \geq \boldsymbol{\epsilon}\big] \nonumber \\
    &\leq \sum_{i\in\mathcal{F}\times\mathcal{T}} \mathbb{P}[|{Q_i}|_{\boldsymbol{x}^*} - \mathbb{E}[{Q_i}|_{\boldsymbol{x}^*}]| \geq \epsilon_i] \leq \sum_{i\in\mathcal{F}\times\mathcal{T}} (\Gamma_i)^2 = \norm{\boldsymbol{\Gamma}}_2^2
\end{align}
where the inequality follows by the union bound and the $\Gamma$-concentration property. Similarly, we have
\begin{align}
& \sum_{\hat{\boldsymbol{q}}\in\mathcal{Q}({\boldsymbol{x}^*})^{\text{Leq}}} L\cdot \norm{\mathbb{E}[\boldsymbol{Q}|_{\boldsymbol{x}^*}] - {\boldsymbol{q}}^*}_{1} \cdot \mathbb{P}_{\boldsymbol{Q}|_{\boldsymbol{x}^*}}(\hat{\boldsymbol{q}})  \leq
\sum_{\hat{\boldsymbol{q}}\in\mathcal{Q}({\boldsymbol{x}^*})^{\text{Leq}}} L\cdot\norm{\boldsymbol{\epsilon}}_{1}\cdot \mathbb{P}_{\boldsymbol{Q}|_{\boldsymbol{x}^*}}(\hat{\boldsymbol{q}}) \nonumber \\
&=
L\cdot\norm{\boldsymbol{\epsilon}}_{1}\cdot\mathbb{P}\big[ \boldsymbol{Q}|_{\boldsymbol{x}^*} \leq \mathbb{E}[\boldsymbol{Q}|_{\boldsymbol{x}^*}]  - \boldsymbol{\epsilon}\big]\leq L\cdot\norm{\boldsymbol{\epsilon}}_{1}\cdot \norm{\boldsymbol{\Gamma}}_2^2
\label{eq_prop2_leq_1}
\end{align}
where the first inequality is due to the $\epsilon$-feasibility.

Therefore, combining Eqs. \ref{eq_prop2_leq_0} and \ref{eq_prop2_leq_1} leads to 
\begin{align}
    \sum_{\hat{\boldsymbol{q}}\in\mathcal{Q}({\boldsymbol{x}^*})^{\text{Leq}}} L\cdot\norm{\hat{\boldsymbol{q}} - \boldsymbol{q}^*}_{1} \cdot \mathbb{P}_{\boldsymbol{Q}|_{\boldsymbol{x}^*}}(\hat{\boldsymbol{q}})  \leq L\cdot\big(\norm{\mathbb{E}[\boldsymbol{Q}|_{\boldsymbol{x}^*}]}_1 + \norm{\boldsymbol{\epsilon}}_{1}\big)\cdot \norm{\boldsymbol{\Gamma}}_2^2
\end{align}

\noindent \textbf{(2) Bounds on the summation over} $\mathcal{Q}({\boldsymbol{x}^*})^{\text{Mid}}$:
\begin{align}
    \sum_{\hat{\boldsymbol{q}}\in\mathcal{Q}({\boldsymbol{x}^*})^{\text{Mid}}} L\cdot\norm{\hat{\boldsymbol{q}} - \boldsymbol{q}^*}_{1} \cdot \mathbb{P}_{\boldsymbol{Q}|_{\boldsymbol{x}^*}}(\hat{\boldsymbol{q}}) 
    & \leq \sum_{\hat{\boldsymbol{q}}\in\mathcal{Q}({\boldsymbol{x}^*})^{\text{Leq}}} L\cdot\left(\norm{\hat{\boldsymbol{q}} - \mathbb{E}[\boldsymbol{Q}|_{\boldsymbol{x}^*}]}_{1} + \norm{\mathbb{E}[\boldsymbol{Q}|_{\boldsymbol{x}^*}] - \boldsymbol{q}^*}_{1}\right) \cdot \mathbb{P}_{\boldsymbol{Q}|_{\boldsymbol{x}^*}}(\hat{\boldsymbol{q}}) \nonumber\\
    & \leq \sum_{\hat{\boldsymbol{q}}\in\mathcal{Q}({\boldsymbol{x}^*})^{\text{Mid}}} L\cdot(\norm{\boldsymbol{\epsilon}}_1+\norm{\boldsymbol{\epsilon}}_1 )\cdot \mathbb{P}_{\boldsymbol{Q}|_{\boldsymbol{x}^*}}(\hat{\boldsymbol{q}}) \leq 2L\cdot\norm{\boldsymbol{\epsilon}}_1 
\end{align}


\noindent \textbf{(3) Bounds on the summation over} $\mathcal{Q}({\boldsymbol{x}^*})^{\text{Geq}}$:

Similar to the proof of $\mathcal{Q}({\boldsymbol{x}^*})^{\text{Leq}}$, notice that
\begin{align}
& \sum_{\hat{\boldsymbol{q}}\in\mathcal{Q}({\boldsymbol{x}^*})^{\text{Geq}}} L\cdot \norm{\hat{\boldsymbol{q}} - \mathbb{E}[\boldsymbol{Q}|_{\boldsymbol{x}^*}] }_{1} \cdot \mathbb{P}_{\boldsymbol{Q}|_{\boldsymbol{x}^*}}(\hat{\boldsymbol{q}})  \leq L\cdot\sum_{\hat{\boldsymbol{q}}\in\mathcal{Q}({\boldsymbol{x}^*})^{\text{Geq}}} 
\norm{\boldsymbol{q}^{\text{Max}}}_1 \cdot \mathbb{P}_{\boldsymbol{Q}|_{\boldsymbol{x}^*}}(\hat{\boldsymbol{q}}) \nonumber \\
&=
L\cdot\norm{\boldsymbol{q}^{\text{Max}}}_1\cdot\mathbb{P}\big[ \boldsymbol{Q}|_{\boldsymbol{x}^*} \leq \mathbb{E}[\boldsymbol{Q}|_{\boldsymbol{x}^*}]  - \boldsymbol{\epsilon}\big]\leq L\cdot\norm{\boldsymbol{q}^{\text{Max}}}_1\cdot \norm{\boldsymbol{\Gamma}}_2^2
\label{eq_prop2_leq_3}
\end{align}
Combining Eqs. \ref{eq_prop2_leq_3} and \ref{eq_prop2_leq_1}, we have
\begin{align}
    \sum_{\hat{\boldsymbol{q}}\in\mathcal{Q}({\boldsymbol{x}^*})^{\text{Geq}}} L\cdot\norm{\hat{\boldsymbol{q}} - \boldsymbol{q}^*}_{1} \cdot \mathbb{P}_{\boldsymbol{Q}|_{\boldsymbol{x}^*}}(\hat{\boldsymbol{q}}) 
    & \leq \sum_{\hat{\boldsymbol{q}}\in\mathcal{Q}({\boldsymbol{x}^*})^{\text{Geq}}} L\cdot\left(\norm{\hat{\boldsymbol{q}} - \mathbb{E}[\boldsymbol{Q}|_{\boldsymbol{x}^*}]}_{1} + \norm{\mathbb{E}[\boldsymbol{Q}|_{\boldsymbol{x}^*}] - \boldsymbol{q}^*}_{1}\right) \cdot \mathbb{P}_{\boldsymbol{Q}|_{\boldsymbol{x}^*}}(\hat{\boldsymbol{q}}) \nonumber\\
    &\leq L\cdot\big(\norm{\boldsymbol{q}^{\text{Max}}}_1 + \norm{\boldsymbol{\epsilon}}_{1}\big)\cdot \norm{\boldsymbol{\Gamma}}_2^2
\end{align}

In summary, combining the summation over three mutually exclusive sets, we have:
\begin{align}
    & \left| \mathbb{E}_{\boldsymbol{Q}|_{\boldsymbol{x}^*}}[STT(\boldsymbol{Q}|_{\boldsymbol{x}^*})]- SST(\boldsymbol{q}^*)\right| \leq 2L\cdot\norm{\boldsymbol{\epsilon}}_1  + L\cdot\big(\norm{\mathbb{E}[\boldsymbol{Q}|_{\boldsymbol{x}^*}]}_1  + \norm{\boldsymbol{q}^{\text{Max}}}_1 + 2\norm{\boldsymbol{\epsilon}}_{1}\big)\cdot \norm{\boldsymbol{\Gamma}}_2^2
\end{align}




% Without loss of generality, we assume $\Psi = 0$ in this proof. For simplicity, we re-write the system travel time $WT(\boldsymbol{Q},z) + IVT()$ as a linear function of $(\boldsymbol{{q}, {z}, {x}})$, that is:




% Consider the problem of expected system travel time:
% \begin{align}
%     a=1
% \end{align}






% Denote the feasible space of Eq. \ref{eq_ipr} as $\Omega = \{(\boldsymbol{{q}, {z}, {x}}):\; \text{Constraints } (\ref{const_IRR0}) - (\ref{const_IRR2})\}$. Since Eq. \ref{eq_ipr} is an integer linear programming, solving it is equivalent to solve an linear programming over its convex hull $\texttt{Conv}(\Omega)$. According to the Minkowski’s Theorem \citep{boyd2004convex}, $\texttt{Conv}(\Omega)$ can be expressed as linear combinations of its extreme points and rays, that is:
% \begin{align}
%     \texttt{Conv}(\Omega) = \{\sum_{(\boldsymbol{{q}, {z}, {x}})\in\mathcal{E}} \boldsymbol{\xi}^T(\boldsymbol{{q}, {z}, {x}}) + \sum_{(\boldsymbol{\tilde{q}, \tilde{z}, \tilde{x}})\in\tilde{\mathcal{E}}} \tilde{\boldsymbol{\xi}}^T(\boldsymbol{\tilde{q}, \tilde{z}, \tilde{x}}):\; \forall \boldsymbol{\xi} \geq 0, \boldsymbol{1}^T\boldsymbol{\xi} = 1,  \forall \tilde{\boldsymbol{\xi}}\geq 0 \}
% \end{align}
% where $\mathcal{E}$ and $\tilde{\mathcal{E}}$ are the sets of extreme points and rays of $\texttt{Conv}(\Omega)$, respectively. $\boldsymbol{1}$ is a vector with all elements equal to 1. $\boldsymbol{\xi}$ and $\tilde{\boldsymbol{\xi}}$ are scalars for linear combinations.

% Hence, the feasible region 

  
% \begin{align}
%     STT(\boldsymbol{q},\boldsymbol{z},\boldsymbol{x}) = \boldsymbol{\varphi}_1^T \boldsymbol{q} + \boldsymbol{\varphi}_2^T \boldsymbol{z} + \boldsymbol{\varphi}_3^T \boldsymbol{x} \label{eq_prop2_stt1}
% \end{align}
% where $\boldsymbol{\varphi}_1,\boldsymbol{\varphi}_2,\boldsymbol{\varphi}_3$ are parameters for the linear expression. Therefore, Eq. \ref{eq_ipr} is equivalent to:
% \begin{align}
%     \min_{(\boldsymbol{{q}, {z}, {x}})\in\texttt{Conv}(\Omega)} STT(\boldsymbol{q},\boldsymbol{z},\boldsymbol{x}) =\boldsymbol{\varphi}_1^T \boldsymbol{q} + \boldsymbol{\varphi}_2^T \boldsymbol{z} + \boldsymbol{\varphi}_3^T \boldsymbol{x} \label{eq_ipr_mik}
% \end{align}
% On the other hand, if we solve the problem with expectation. The formulation is
% \begin{align}
%       \min_{(\boldsymbol{\mathbb{E}{[Q]}, {z}, {x}})\in\texttt{Conv}(\Omega^{\text{Exp}})} \mathbb{E}[STT(\boldsymbol{Q},\boldsymbol{z},\boldsymbol{x})] =\boldsymbol{\varphi}_1^T \mathbb{E}[\boldsymbol{Q}] + \boldsymbol{\varphi}_2^T \boldsymbol{z} + \boldsymbol{\varphi}_3^T \boldsymbol{x} \label{eq_ipr_mik} 
% \end{align}
% where $\Omega^{\text{Exp}}$ is same as $\Omega$ except for replacing all $\boldsymbol{q}$ with $\mathbb{E}{[\boldsymbol{Q}]}$. This is because any linear constraint with expectation can be expressed as:
% \begin{align}
%     \mathbb{E}[\boldsymbol{a}^T(\boldsymbol{Q},\boldsymbol{z},\boldsymbol{x})] \leq \boldsymbol{b} \Longleftrightarrow \boldsymbol{a}^T(\mathbb{E}[\boldsymbol{Q}],\boldsymbol{z},\boldsymbol{x}) \leq \boldsymbol{b} \label{eq_prop2_3}
% \end{align}
% Eq. \ref{eq_prop2_3} implies that we can simply replacing $\boldsymbol{q}$ with $\mathbb{E}[\boldsymbol{Q}]$ in Eq. \ref{eq_prop2_stt1} to obtain Eq. \ref{eq_ipr_mik}

% Let $(\boldsymbol{{q}^*, {z}^*, {x}^*})$ be the optimal solution of Eq. \ref{eq_ipr_mik}. Then the model-evaluated system travel time is $STT(\boldsymbol{q}^*,\boldsymbol{z}^*,\boldsymbol{x}^*) = \boldsymbol{\varphi}_1^T \boldsymbol{q}^* + \boldsymbol{\varphi}_2^T \boldsymbol{z}^* + \boldsymbol{\varphi}_3^T \boldsymbol{x}^*$. 


% Given $\boldsymbol{q}^*$, let the associated random variable be $\boldsymbol{Q}^*$. Then, the expected system travel time is
% \begin{align}
%     \mathbb{E}[STT(\boldsymbol{Q}^*,\boldsymbol{z}^*,\boldsymbol{x}^*)] = \boldsymbol{\varphi}_1^T \mathbb{E}[\boldsymbol{Q}^*] + \boldsymbol{\varphi}_2^T \boldsymbol{z}^* + \boldsymbol{\varphi}_3^T \boldsymbol{x}^*
% \end{align}
% Hence, the difference between model-evaluated and expected $STT$ is
% \begin{align}
%   & |\mathbb{E}(STT(\boldsymbol{Q}^*,\boldsymbol{z}^*,\boldsymbol{x}^*)) - STT(\boldsymbol{q}^*,\boldsymbol{z}^*,\boldsymbol{x}^*)| \nonumber \\
%     &= \sum_{i={(u,v,r,t)}\in\mathcal{F}\times\mathcal{T}}{\varphi}_{1,i}\cdot(|\mathbb{E}[Q_i^*] - q_i^*|) \leq \sum_{i={(u,v,r,t)}\in\mathcal{F}\times\mathcal{T}}{\varphi}_{1,i}\cdot \epsilon \label{eq_prop2_eq2}
% \end{align}
% Eq. \ref{eq_prop2_eq2} holds for all possible optimal solutions. The set of all possible optimal solutions is in the extreme points set (assuming the problem is bounded). Hence, a general bound for the difference is:
% \begin{align}
%  |\mathbb{E}(STT(\boldsymbol{Q}^*,\boldsymbol{z}^*,\boldsymbol{x}^*)) - STT(\boldsymbol{q}^*,\boldsymbol{z}^*,\boldsymbol{x}^*)| \
% \end{align}
% where 
% is a linear combination of extreme points and rays .  Then there exist $\boldsymbol{\xi}^*$ and $\tilde{\boldsymbol{\xi}}^*$ where such that
% \begin{align}
%     (\boldsymbol{{q}^*, {z}^*, {x}^*}) = 
% \end{align}
% The optimal objective function can be expressed as
% \begin{align}
%     \boldsymbol{\varphi}_1^T \boldsymbol{q} + \boldsymbol{\varphi}_2^T \boldsymbol{z} + \boldsymbol{\varphi}_3^T \boldsymbol{x}
% \end{align}
